Krylov Subspace Recycling for Sequences of Shifted Linear Systems

We study the use of Krylov subspace recycling for the solution of a sequence of slowly-changing families of linear systems, where each family consists of shifted linear systems that differ in the coefficient matrix only by multiples of the identity. Our aim is to explore the simultaneous solution of each family of shifted systems within the framework of subspace recycling, using one augmented subspace to extract candidate solutions for all the shifted systems. The ideal method would use the same augmented subspace for all systems and have fixed storage requirements, independent of the number of shifted systems per family. We show that a method satisfying both requirements cannot exist in this framework. As an alternative, we introduce two schemes. One constructs a separate deflation space for each shifted system but solves each family of shifted systems simultaneously. The other builds only one recycled subspace and constructs approximate corrections to the solutions of the shifted systems at each cycle of the iterative linear solver while only minimizing the base system residual. At convergence of the base system solution, we apply the method recursively to the remaining unconverged systems. We present numerical examples involving systems arising in lattice quantum chromodynamics.

==> multi-defl-spaces.tex <==
%\def\thesection{\alpha{section}}
%\appendix
\subsection{Constructing Multiple Deflation Spaces}
We now return to the question of constructing multiple deflation spaces.  
\linespread{1}%set to single spacing for the algorithm so it is more compact
\begin{algorithm}[b!]
\caption{Computing a Family of Recycled Spaces for Multiple Shifted Linear Systems}
\label{alg.multi-shift-recycle-space}
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\Input{$\vek A\in\C^{n\times n}$, $\curl{\sigma_{i}}_{i=1}^{s+1}\subset\C$, $\widetilde{\vek U}\in\C^{n\times k}$}
\Output{$\vek C\in\C^{n\times k}$ such that $\vek C^{\ast}\vek C = \vek I_{k}$, $\curl{\vek U^{(\sigma_{i})}}_{i=1}^{s+1}$ such that $(\vek A + \sigma_{i}\vek I)\vek 
U^{(\sigma_{i})} = \vek C$ for all $i$}
\For{$i=1$ to $s+1$}{
	$\vek U^{(\sigma_{i})} = \widetilde{\vek U}$\\
}

\For{$i=1$ to $s$}{
	$\vek U^{(\sigma_{s+1})} \leftarrow \vek A\vek U^{(\sigma_{s+1})} + \sigma_{i}\vek U^{(\sigma_{s+1})}$\\
	Compute the QR-factorization $\vek U^{(\sigma_{s+1})} = \vek Q\vek R$\\
	$\vek U^{(\sigma_{s+1})} \leftarrow \vek Q$\\
	\For{$j=1$ to $s$}{
		$\widehat{\vek U} \leftarrow \vek U^{(\sigma_{j})}\vek R^{-1}$\\
		$k_{1} \leftarrow (j-1\mod s+1) + (1-\ceil{\frac{j-1}{s+1}})(s+1)$\\
		$k_{2} \leftarrow (j+1\mod s+1) + \floor{\frac{j+1}{s+1}}(s+1)$\\
		 $\vek U^{(\sigma_{j})} \leftarrow \vek U^{(\sigma_{k_{1}})} + (\sigma_{k_{2}} - \sigma_{j})\widehat{\vek U}$
	}
}
$\vek C = \vek A\vek U^{(\sigma_{s+1})} + \sigma_{s+1}\vek U^{(\sigma_{s+1})}$ \\
Compute the QR-factorization $\vek C=\vek Q\vek R$\\
$\vek C \leftarrow \vek Q$\\
\For{$i=1$ to $s+1$}{
	$\vek U^{(\sigma_{i})} \leftarrow \vek U^{(\sigma_{i})}\vek R^{-1}$
}
\end{algorithm}
Given a matrix $\widetilde{\vek U}\in\C^{n\times k}$ with columns spanning our recycled space, how do we compute $
\vek U$ and $\vek U^{(\sigma)}$ such that both 
%\begin{figure}[htb]
%%\begin{center}
%\hfill
%\includegraphics[scale=0.35]{figures/shiftedRecycleSpaceFig.eps}
%\hfill
%%\begin{picture}(0,0)
%%\put(-120,144){{\footnotesize Base System}}
%%\end{picture}
%%\vspace*{2em}
%%\end{center}
%\caption{The performance of Algorithm \ref{alg.multi-shift-recycle-space} for a collection of shifts taken from the interval $\brac{10^{-8},10^{8}}$.  For this figure, both 
%axes are on a logarithmic scale. We compute the largest principal angle between $\CR(\vek C)$ and $\CR((\vek A+\sigma\vek I)\vek U^{(\sigma)})$ to examine the 
%accuracy. \textbf{Observe} that there is an increase in accuracy for the right-most shift, $\sigma=10^{8}$.  The subspace associated to $\sigma=10^{8}$
% corresponds to 
%$\vek U^{(\sigma_{s+1})}$ in Algorithm \ref{alg.multi-shift-recycle-space}. The computation of $\vek U^{(\sigma_{s+1})}$
% is done directly rather than by using Proposition \ref{prop.many-prod-one-matvec}.}
%\label{figure.shifted-recycle-space}
%\end{figure}
\begin{equation}\label{eqn.AUUsig}
	\vek A\vek U = \vek C \mbox{\ \ \ and\ \ \ } (\vek A + \sigma\vek I)\vek U^{(\sigma)} = \vek C\mbox{\ \ with\ \ }\vek C^{\ast}\vek C=\vek I?
\end{equation}
In \RGMRES, we compute $\vek A\widetilde{\vek U} = \widetilde{\vek C}$ at the cost of one block matrix-vector
product.  
\begin{figure}[htb!]
\hfill
\includegraphics[scale=0.60]{shiftedRecycleSpaceFigAllRads.eps}
\hfill 
\begin{picture}(0,0)

%left top figure
%\put(119,275){{\footnotesize $10$}}
%\put(170,275){{\footnotesize $10.1$}}
%\put(67,275){{\footnotesize $9.9$}}

%left middle figure
\put(-291,145){{\footnotesize $0$}}
\put(-251,145){{\footnotesize $10$}}
\put(-205,145){{\footnotesize $20$}}

%left bottom figure
\put(-298,21){{\footnotesize $-90$}}
\put(-251,21){{\footnotesize $10$}}
\put(-205,21){{\footnotesize $110$}}

%right top figure
%\put(329,160){{\footnotesize $10^{5}$}}
%\put(275,160){{\footnotesize $1.1\times 10^{5}$}}
%\put(220,160){{\footnotesize $9.9\times 10^{4}$}}

%right middle figure
\put(-141,145){{\footnotesize $0$}}
\put(-106,145){{\footnotesize $2\times10^{5}$}}
\put(-55,145){{\footnotesize $10^{5}$}}

%right bottom figure
\put(-146,21){{\footnotesize $9.9\times 10^{5}$}}
\put(-101,21){{\footnotesize $10^{5}$}}
\put(-55,21){{\footnotesize $1.1\times 10^{6}$}}

%the gammas
%\put(115,343){{\footnotesize $\gamma = 10^{-1}$}}
\put(-115,228){{\footnotesize $\gamma=10^{5}$}}
\put(-115,105){{\footnotesize $\gamma=10^{6}$}}
%\put(263,343){{\footnotesize $\gamma=10^{4}$}}
\put(-263,228){{\footnotesize $\gamma=10$}}
\put(-270,106){{\footnotesize $\gamma=10^{2}$}}

\end{picture}
%\vspace*{2em}
%\end{center}
\caption{The performance of Algorithm \ref{alg.multi-shift-recycle-space} for collections of shifts.  Different lines depict the algorithm's performance for different 
numbers of shifts.  Line darkness increases when more shifts are used (meaning the algorithm requires more iterations). We compute the largest principal angle 
between $\CR(\vek C)$ and $\CR((\vek A+\sigma\vek I)\vek U^{(\sigma)})$ to examine the accuracy.  In the figures in the left column, shifts come from the interval $
\brac{10-\gamma,10+\gamma}$.  In the right column, shifts come from the interval $\brac{10^{5}-\gamma,10^{5}+\gamma}$.  Observe that the Algorithm 
\ref{alg.multi-shift-recycle-space} performs well for larger values of $\gamma$ when the center is located at $10^{5}$.}
\label{figure.shfited-recycle-space-dist}
\end{figure}
Can we achieve (\ref{eqn.AUUsig}) with only two block matrix-vector products? 

Suppose we have two coefficient matrices $\vek A$ and $(\vek A + \sigma \vek I)$.  
To get a pair of matrices $\vek U$ and $\vek U^{(\sigma)}$ 
satisfying (\ref{eqn.AUUsig}), we premultiply $\widetilde{\vek U}$ by both $
\vek A$ and $\vek A+\sigma\vek I$.  In other words, 
let $\widetilde{\vek C} = \vek A(\vek A + \sigma\vek I)\widetilde{\vek U}$ and compute the QR-factorization  $
\widetilde{\vek C} = \vek C\vek R$.  Then we have 
$\vek U = (\vek A + \sigma\vek I)\widetilde{\vek U}\vek R^{-1}$ and $\vek U^{(\sigma)} = \vek A\widetilde{\vek U}
\vek R^{-1}$.  Since matrices differing  by multiples of the identity commute, 
we have $\vek A\vek U = (\vek A+\sigma\vek I)\vek U^{(\sigma)} = \vek C$.  This easily 
can be generalized to any number of shifts.  Given a sequence of 
shifts $\curl{\sigma^{i}}_{i=1}^{s+1}\subset\C$, where we consider the base matrix as a system with 
shift $\sigma_{1}=0$, the matrices 
\[
	\vek U^{(\sigma_{j})} = \brac{\prod_{i=1,i\neq j}^{s+1}(\vek A+\sigma_{i})}\widetilde{\vek U}\vek R^{-1} \mbox{\ \ \ and\ \ \ } \vek C = \brac{\prod_{i=1}^{s+1}(\vek A
+\sigma_{i})}\widetilde{\vek U}\vek R^{-1} 
\]
satisfy our requirements with $\widetilde{\vek C} = \vek C\vek R$ being the 
QR-factorization of $\widetilde{\vek C}$.  
We have that $(\vek A + \sigma_{i}\vek I)\vek U^{(\sigma_{i})} = \vek C$ for all $i$.  
This strategy has clear stability issues which must be addressed.  
Furthermore, we wish to execute as few calls to the operator $\vek A$ as possible. 
Therefore, we propose a  more stable implementation of this procedure.

Though these matrices do commute, once we choose a particular multiplication 
order, e.g., if $\vek C = \vek A(\vek A+\sigma\vek I)\widetilde{\vek U}\vek R^{-1}$, we 
must proceed intelligently to recover $\vek U^{(\sigma)}~=~\vek A\widetilde{\vek U}\vek R^{-1}$ 
without doing additional matrix vector products.  To address this 
issue, we first introduce a straightforward proposition whose proof follows by simple algebraic manipulation.
\begin{proposition}\label{prop.many-prod-one-matvec}
	Let $\widehat{\vek U} = (\vek A+\sigma_{1}\vek I)\widetilde{\vek U}$.  
	Then $(\vek A+\sigma_{2}\vek I)\widetilde{\vek U} = \widehat{\vek U} + (\sigma_{2}~-~
\sigma_{1})\widetilde{\vek U}$.  Furthermore, let $\widehat{\vek U} = \vek C\vek R$ be the QR-factorization.  Then 
\[
	(\vek A+\sigma_{2}\vek I)\widetilde{\vek U}\vek R^{-1}~=~\vek C~+~(\sigma_{2}-\sigma_{1})\widetilde{\vek U}\vek R^{-1}.
\]
\end{proposition}

For clarity, we present a small example to motivate a general algorithm for this process.  
Suppose we have three shifted systems $\vek A+\sigma_{1}\vek I
$, $\vek A+\sigma_{2}\vek I$, and $\vek A+\sigma_{3}\vek I$.  Given 
$\widehat{\vek U}\in\C^{n\times k}$, how do we generate $\vek U^{(\sigma_{1})},\vek 
U^{(\sigma_{2})},\vek U^{(\sigma_{3})}\in\C^{n\times k}$ such that for some 
$\vek C\in\C^{n\times k}$ such that $\vek C^{\ast}\vek C = \vek I_{k}$, we have 
\[
	(\vek A+\sigma_{1}\vek I)\vek U^{(\sigma_{1})} = \vek C\mbox{\ \ \ and\ \ \ } (\vek A+\sigma_{2}\vek I)\vek U^{(\sigma_{2})} = \vek C \mbox{\ \ \ and\ \ \ } (\vek A+
\sigma_{3}\vek I)\vek U^{(\sigma_{3})} = \vek C.
\]
Furthermore, we want to do this using three block $k$ 
matrix-vector products and $k$-dimensional basis orthogonalizations.  
This is a three-step process, and at each step, we will 
apply a shifted operator once and use Proposition 
\ref{prop.many-prod-one-matvec} to implicitly 
Let 
\[
	\vek U^{(\sigma_{1})}_{0} = \vek U^{(\sigma_{2})}_{0} = \vek U^{(\sigma_{3})}_{0} = \widehat{\vek U}.
\]
We first compute $\widehat{\vek U}^{(\sigma_{3})}_{1} = (\vek A+\sigma_{1}\vek I)\vek 
U^{(\sigma_{2})}_{0}$ and the QR-factorization $\widehat{\vek U}^{(\sigma_{3})}_{1} = \vek U^{(\sigma_{3})}_{1}\vek R_{1}$. By  Proposition \ref{prop.many-prod-one-matvec}, we know that 
\begin{equation}\label{eqn.Usig1to3}
	\vek U^{(\sigma_{1})}_{1} = \vek U^{(\sigma_{3})}_{1} + (\sigma_{2} - \sigma_{1})\vek U^{(\sigma_{1})}_{0}\vek R^{-1}_{1}
\end{equation}
which then implies that, again by Proposition \ref{prop.many-prod-one-matvec},
\[
	\vek U^{(\sigma_{2})}_{1} = \vek U^{(\sigma_{1})}_{1} + (\sigma_{3} - \sigma_{2})\vek U^{(\sigma_{2})}_{0}\vek R^{-1}_{1}.
\]
Next, we compute $\widehat{\vek U}^{(\sigma_{3})}_{2} = (\vek A+\sigma_{2}\vek I)\vek 
U^{(\sigma_{2})}_{1}$ and the QR-factorization $\widehat{\vek U}^{(\sigma_{3})}_{2} = \vek U^{(\sigma_{3})}_{2}\vek R_{2}$. Then we have
\begin{eqnarray}
 \widehat{\vek U}^{(\sigma_{1})}_{2}& = & (\vek A+\sigma_{3}\vek I)\vek U^{(\sigma_{1})}_{1}\label{eqn.Uprods2}\\
 & = &(\vek A+\sigma_{3}\vek I)(\vek U^{(\sigma_{3})}_{1} + (\sigma_{2} - \sigma_{1})\vek U^{(\sigma_{1})}_{0}\vek R^{-1}_{1})\nonumber\\
 & = &(\vek A+\sigma_{2}\vek I)\vek U^{(\sigma_{3})}_{1} + (\sigma_{3}-\sigma_{2})\vek U^{(\sigma_{3})}_{1} + (\sigma_{2} - \sigma_{1})(\vek A+\sigma_{3}\vek I)\vek 
U^{(\sigma_{1})}_{0}\vek R^{-1}_{1} \nonumber \\
 & = & \widehat{\vek U}^{(\sigma_{3})}_{2} + (\sigma_{3}-\sigma_{2})\vek U^{(\sigma_{3})}_{1} + (\sigma_{2} - \sigma_{1})(\vek A+\sigma_{3}\vek I)\vek 
U^{(\sigma_{1})}_{0}\vek R^{-1}_{1}.\nonumber
\end{eqnarray}
By Proposition \ref{prop.many-prod-one-matvec},  
\[
	(\vek A+\sigma_{3}\vek I)\vek U^{(\sigma_{1})}_{0}\vek R^{-1}_{1} = {\vek U^{(\sigma_{3})}_{1} + (\sigma_{3}-\sigma_{1})\vek U^{(\sigma_{1})}_{0}\vek R^{-1}
_{1}},
\]
yielding
\begin{eqnarray}
 \widehat{\vek U}^{(\sigma_{1})}_{2} & = &  \widehat{\vek U}^{(\sigma_{3})}_{2} + (\sigma_{3}-\sigma_{2})\vek U^{(\sigma_{3})}_{1} + (\sigma_{2} - \sigma_{1})({\vek 
U^{(\sigma_{3})}_{1} + (\sigma_{3}-\sigma_{1})\vek U^{(\sigma_{1})}_{0}\vek R^{-1}_{1}}) \nonumber\\
 & = &  \widehat{\vek U}^{(\sigma_{3})}_{2} + (\sigma_{3}-\sigma_{2})\vek U^{(\sigma_{3})}_{1} + (\sigma_{2} - \sigma_{1}){\vek U^{(\sigma_{3})}_{1} + (\sigma_{2} - 
\sigma_{1})(\sigma_{3}-\sigma_{1})\vek U^{(\sigma_{1})}_{0}\vek R^{-1}_{1}}  \nonumber\\
 & = &  \widehat{\vek U}^{(\sigma_{3})}_{2} + (\sigma_{3}-\sigma_{2})\vek U^{(\sigma_{3})}_{1} + (\sigma_{2} - \sigma_{1}){\vek U^{(\sigma_{3})}_{1} + (\sigma_{2} - 
\sigma_{1})(\sigma_{3}-\sigma_{1})\vek U^{(\sigma_{1})}_{0}\vek R^{-1}_{1}} \nonumber \\
 & = &  \widehat{\vek U}^{(\sigma_{3})}_{2} + (\sigma_{3}-\sigma_{1})\vek U^{(\sigma_{3})}_{1} + (\sigma_{2} - \sigma_{1})(\sigma_{3}-\sigma_{1})\vek 
U^{(\sigma_{1})}_{0}\vek R^{-1}_{1} \nonumber \\
 & = &  \widehat{\vek U}^{(\sigma_{3})}_{2} + (\sigma_{3}-\sigma_{1})(\vek U^{(\sigma_{3})}_{1} + (\sigma_{2} - \sigma_{1})\vek U^{(\sigma_{1})}_{0}\vek R^{-1}_{1}). 
\nonumber
\end{eqnarray}
Finally, by (\ref{eqn.Usig1to3}), we have that 
\[
	\widehat{\vek U}^{(\sigma_{1})}_{2} =  \widehat{\vek U}^{(\sigma_{3})}_{2} + (\sigma_{3}-\sigma_{1})\vek U^{(\sigma_{1})}_{1},
\]
which, when we post multiply by $\vek R_{2}^{-1}$, gives us
\[
	{\vek U}^{(\sigma_{1})}_{2} ={\vek U}^{(\sigma_{3})}_{2} + (\sigma_{3}-\sigma_{1})\vek U^{(\sigma_{1})}_{1}\vek R_{2}^{-1}.
\]
A similar derivation shows us that 
\[
	{\vek U}^{(\sigma_{2})}_{2} ={\vek U}^{(\sigma_{1})}_{2} + (\sigma_{1}-\sigma_{2})\vek U^{(\sigma_{2})}_{1}\vek R_{2}^{-1}.
\]
From here, we can compute the QR-factorization 
$(\vek A + \sigma_{3}\vek I){\vek U}^{(\sigma_{3})}_{2} = \vek C\vek R_{3}$ and let
\[
	\vek U^{(\sigma_{1})} = \vek U^{(\sigma_{1})}_{2}\vek R_{3}^{-1}\mbox{\ \ \ and\ \ \ } \vek U^{(\sigma_{2})} = \vek U^{(\sigma_{2})}_{2}\vek R_{3}^{-1} \mbox{\ \ \ 
and\ \ \ } \vek U^{(\sigma_{3})} = \vek U^{(\sigma_{3})}_{2}\vek R_{3}^{-1}.
\]

For the general case, in which we have $s+1$ shifts, this suggests 
an \linebreak$(s+1)$-step algorithm for the computation $\vek U^{(\sigma_{i})}$ for all $i$ and $
\vek C$ such that $\vek C^{\ast}\vek C = \vek I_{k}$.    We begin with some notation.  
For any shift $\sigma_{i}$, $\vek U^{(\sigma_{i})}$ is such that $(\vek A~+~
\sigma_{i}\vek I)\vek U^{(\sigma_{i})}=\vek C$.    At the $j$th step, we compute $k$ 
matrix-vector products and generate an intermediate matrix $\vek U^{(\sigma_{i})}
_{j}$ for each shift, and we denote the initial recycled space associated 
to $\sigma_{i}$, $\vek U_{0}^{(\sigma_{i})} = \widetilde{\vek U}$.  At step $j$, we compute the 
product 
\[
	\widehat{\vek U}_{j}^{(\sigma_{i})}~=~(\vek A + \sigma_{\rho_{j}}\vek I)\vek U_{j-1}^{(\sigma_{i})}, 
\]
where $\rho_{j} = (j+1\mod s+1) + \floor{\frac{j+1}{s+1}}(s+1)$.  This formula 
for $\rho_{j}$ allows us to cyclically index through all the shifts using arithmetic on the 
group $\Z_{s+1}=\curl{1,2,\ldots,s+1}$.  For stability, we need to maintain orthogonality
 of one of the bases.  Therefore, without loss 
of generality, we compute the QR-factorization $\widehat{\vek U}_{j}^{(\sigma_{s+1})}~=~\vek U_{j}^{(\sigma_{s+1})}\vek R_{j}$ and update $\vek U_{j}^{(\sigma_{i})} 
= \widehat{\vek U}_{j}^{(\sigma_{i})}\vek R_{j}^{-1}$ for each $i \neq s+1$.  In each step of this process, we only 
compute one block $k$ matrix-vector product explicitly (associated to $\sigma_{s+1}$).  
The others are computed using Proposition \ref{prop.many-prod-one-matvec}.  
At the end of the process, we have  computed 
$s$ block $k$ matrix-vector products.  We finish by 
computing $\widehat{\vek C} = (\vek A + \sigma_{s+1}\vek I)\vek U_{s}
^{(\sigma_{s+1})}$ and one final QR-factorization $\widehat{\vek C} = \vek C\vek R$.  
We then update $\vek U^{(\sigma_{i})} = \vek U_{s}^{(\sigma_{i})}\vek R^{-1}$ 
for all~$i$.  We present these steps more precisely in Algorithm \ref{alg.multi-shift-recycle-space}. 

In the computation of these subspaces, 
we must choose one shift for which we will compute $\vek U^{(\sigma)}$ directly.  
Then we use Proposition \ref{prop.many-prod-one-matvec} 
to implicitly do the other computations.  We chose the rightmost shift to be the one for which we explicitly do 
the computations.  Thus, we get a much smaller principal angles for the subspace associated to the last shift.  
It's not affected by any numerical errors are causing the algorithm's performance degradation 
for the other shifts.  Experimentally, we observe that 
three other criteria on the set of shifts also seem to affect the stability of the 
algorithm.  For a collection of real shifts, let $\curl{\sigma_{i}}_{i=1}^{s}\subset\brac{a,b}$ 
with $a < b$ where $\brac{a,b}$ is the smallest interval containing all shifts.  
We have observed that $\ab{b-a}$ affects stability.  However, this effect is relative to 
the distance of the set of shifts from the origin, where 
we define distance as $\ab{b+a}/2$, the distance of the midpoint from the origin.  
The further the distance of the set from the origin, the larger $\ab{b-a}$ can be 
before instability onsets.  
What determines the performance of Algorithm \ref{alg.multi-shift-recycle-space} is 
how closely clustered the shifts are, where ``close'' is defined relative to the 
distance of the midpoint from the origin.  Again, we see the drop in principal angle magnitude for the rightmost shift.

Suppose that the initial recycled space $\widetilde{\vek U}$ is an approximate invariant 
subspace of $\vek A$ associated to small-magnitude eigenvalues. The process 
described in Algorithm \ref{alg.multi-shift-recycle-space} might yield a matrix $\vek C$ with 
columns spanning a new approximate invariant subspace.  This new 
subspace might not be associated to small magnitude eigenvalues, though.  
Because $\vek C$ is constructed implicitly by premultiplying $\widetilde{\vek U}$ by 
different members of the family of shifted matrices, it is not clear what eigenspace $\CR(\vek C)$ might approximate. 

